Rees Algebras of Unit Interval Determinantal Facet Ideals

Using SAGBI basis techniques, we find Gr\"obner bases for the presentation ideals of the Rees algebras and special fiber rings of unit interval determinantal facet ideals. In particular, we show that unit interval determinantal facet ideals are of fiber type and that their special fiber rings are Koszul. Moreover, their Rees algebras and special fiber rings are normal Cohen-Macaulay domains and have rational singularities.

==> notFiberType.tex <==
\begin{figure}[h]
\begin{tikzpicture}[scale=0.80]
\filldraw
(-1.5,0) circle (2.5pt)--
(0,1) circle (2.5pt) --
(0,0) circle (2.5pt)  -- 
(0,-1) circle (2.5pt) --
(1.5,0) circle (2.5pt);
\draw (1.5,0)--(0,1);
\draw (-1.5,0)--(0,-1);
		\node (0) at (0, 1.4) {1};
		\node (1) at (0.4, 0) {2};
		\node (2) at (0, -1.4) {3};
		\node (3) at (1.95, 0) {4};
		\node (4) at (-1.95, -0) {5};
\end{tikzpicture}\caption{A graph corresponding to a binomial edge ideal which is not of fiber type.}\label{fig:nonFiberTypeBEI}
\end{figure}
